Accelerated Gradient Temporal Difference Learning

The family of temporal difference (TD) methods span a spectrum from computationally frugal linear methods like TD({\lambda}) to data efficient least squares methods. Least square methods make the best use of available data directly computing the TD solution and thus do not require tuning a typically highly sensitive learning rate parameter, but require quadratic computation and storage. Recent algorithmic developments have yielded several sub-quadratic methods that use an approximation to the least squares TD solution, but incur bias. In this paper, we propose a new family of accelerated gradient TD (ATD) methods that (1) provide similar data efficiency benefits to least-squares methods, at a fraction of the computation and storage (2) significantly reduce parameter sensitivity compared to linear TD methods, and (3) are asymptotically unbiased. We illustrate these claims with a proof of convergence in expectation and experiments on several benchmark domains and a large-scale industrial energy allocation domain.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{enumitem}


%%%%%%%% Distribution definitions %%%%%%%%%%%%%%%

\newcommand{\normal}{\mathcal{N}}
\newcommand{\given}{|}

%%%%%%%% Matrix/vector definitions %%%%%%%%%%%%%%%

\newcommand{\inlinevec}[2]{%
  \ensuremath{\Bigl[\negthinspace\begin{smallmatrix}#1\\#2\end{smallmatrix}\Bigr]}}
\newcommand{\inlinemat}[4]{%
  \ensuremath{\Bigl[\negthinspace\begin{smallmatrix}#1 \ \ #2 \\#3 \ \ #4\\\end{smallmatrix}\Bigr]}}
\newcommand{\mathvec}[2]{\left[\begin{array}{c}#1\\#2\end{array} \right] }

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}
%\newcommand{\makevector}[1]{{\mathbf #1}}
\newcommand{\zerovec}{\vec{0}}
\newcommand{\onevec}{\vec{1}}
\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\eye}{\mathbf{I}}

%%%%%%%% Simple math functions %%%%%%%%%%%%%%%
\newcommand{\pinv}{\dagger}
\newcommand{\sgrad}{\partial}
\newcommand{\sign}[1]{\mathrm{sign}(#1)}
\newcommand{\posdef}{\succeq}
\newcommand{\e}{{\textrm{e-}}}
\newcommand{\Dom}{{\textrm{Dom}}}
\newcommand{\smallinv}[1]{{#1}^{\scalebox{0.5}[0.5]{\( - 1\)}}}

%%%%%%%% Norm definitions %%%%%%%%%%%%%%%
\newcommand{\frob}[1]{\left\| #1 \right\|_F}
\newcommand{\frobsq}[1]{\left\| #1 \right\|_F^2}
\newcommand{\frobsqtr}[1]{\text{tr}\left(#1'#1\right)}
\newcommand{\sqnorm}[1]{\Big\|  #1 \Big\|_{2}}
\newcommand{\spnorm}[1]{\left\|  #1 \right\|_{sp}}
\newcommand{\tracenorm}[1]{\left\|  #1 \right\|_{tr}}
\newcommand{\twonorm}[1]{\left\|  #1 \right\|_2}
\newcommand{\twoone}[1]{\left\|  #1 \right\|_{2,1}}
\newcommand{\bregman}[3]{D_{#1}(#2 \; || \: #3)}

%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % RR numbers
\newcommand{\RRbar}{\overline{\RR}} % RR numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

% Set of [0, infty]
\newcommand{\RRpos}{{\RR^+}}

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\col}{\mathop{\mathrm{col}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\eigs}{\mathop{\mathrm{eigs}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\nulls}{\mathop{\mathrm{null}}}
\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\row}{\mathop{\mathrm{row}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\spec}{\mathop{\mathrm{sp}}}
\newcommand{\sspan}{{\textrm{span}}}
\newcommand{\svd}{\mathop{\mathrm{svd}}}
\newcommand{\te}{\mathop{\mathrm{te}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\DeclareMathOperator\arctanh{arctanh}
%\newcommand{\ln}{\mathop{\mathrm{ln}}}

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
\newcommand{\set}[2]{\{#1 \ | \ #2\}}
\newcommand{\subfigurespace}[1]{ % Reasonable value = 0.1
\begin{minipage}[b]{#1\textwidth}
 \textbf{ }
 \end{minipage}}
 \newcommand{\figspace}{\begin{minipage}[b]{0.1\textwidth} \textbf{ } \end{minipage}}
\newcommand{\unaryminus}{\scalebox{0.75}[1.0]{\( - \)}}

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}


%%%%%%%% Text definitions %%%%%%%%%%%%%%%

\newcommand{\apriori}{{\emph{a priori}}}
\newcommand{\emphdef}[1]{\textbf{#1}}
\newcommand{\introword}[1]{\textbf{\emph{#1}}}
\newcommand{\emphstart}[1]{\textbf{#1}}
\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\text{i.i.d.}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }
\newcommand{\subheader}[1]{
\vspace{8pt}
\noindent
{\large\bfseries #1}}

%%%%%%%% Examples of Stock standard definitions %%%%%%%%%%%%%%%
% This is just here as a reference for naming convention

%\newcommand{\xb}{\mathbf{x}}
%\newcommand{\xbtil}{\tilde{\xb}}
%\newcommand{\xtil}{\tilde{x}}
%\newcommand{\xhat}{\hat{x}}
%\newcommand{\xbhat}{\hat{\xb}}
%\newcommand{\Xtil}{\tilde{X}}
%\newcommand{\xbar}{\bar{x}}
%\newcommand{\xbbar}{\bar{\xb}}
%\newcommand{\Xb}{\mathbf{X}}
%\newcommand{\Xbtil}{\tilde{\Xb}}
%\newcommand{\Xbar}{\bar{X}}
%\newcommand{\Xbbar}{\bar{\Xb}}
%\newcommand{\Xhat}{\hat{X}}
%\newcommand{\Xbhat}{\hat{\Xb}}
%\newcommand{\Xcal}{\mathcal{X}}
%\newcommand{\Xtilde}{\widetilde{X}}
%\newcommand{\xvec}{\vec{x}}
%\newcommand{\Xvec}{\vec{X}}
%\newcommand{\xvecbar}{\bar{\vec{x}}}
%\newcommand{\xvechat}{\hat{\vec{x}}}
%\newcommand{\valhat}{\hat{\val}}

%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\newcommand{\eproof}{$\null\hfill\blacksquare$}
%\ifx\proof\undefined
\renewenvironment{proof}{\par\noindent{\bf Proof:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
\newenvironment{proofsketch}{\par\noindent{\bf Proof Sketch:\ }}{\eproof} %{\hfill\BlackBox\\[.3mm]}
%\fi
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}

% If end proof with align, then can add a negative space to bring up proof box
\newcommand{\palignbox}{\par \vspace{-0.8cm}}

\newif\ifsamenumbers

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\ifsamenumbers
\newtheorem{lemma}[theorem]{Lemma}
\else
\newtheorem{lemma}{Lemma}
\fi
\fi

\ifx\proposition\undefined
\ifsamenumbers
\newtheorem{proposition}[theorem]{Proposition}
\else
\newtheorem{proposition}{Proposition}
\fi
\fi

\ifx\remark\undefined
\newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
\ifsamenumbers
\newtheorem{corollary}[theorem]{Corollary}
\else
\newtheorem{corollary}{Corollary}
\fi
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\ifsamenumbers
\newtheorem{conjecture}[theorem]{Conjecture}
\else
\newtheorem{conjecture}{Conjecture}
\fi
\fi

\ifx\axiom\undefined
\newtheorem{axiom}{Axiom}
\fi

\ifx\claim\undefined
\ifsamenumbers
\newtheorem{claim}[theorem]{Claim}
\else
\newtheorem{claim}{Claim}
\fi
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}
\newcommand{\myintertext}[1]{\end{enumerate} #1\begin{enumerate}[resume]}
\newenvironment{cenumerate}{%
\vspace{10pt}
\noindent{\Large\bfseries Contributions:}
\begin{enumerate}[label={\textbf{Contribution \arabic*.}\ },leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
}
{\end{enumerate}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}
\newcommand{\pca}{\text{\sc pca}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


